Asking without Telling: Exploring Latent Ontologies in Contextual Representations

The success of pretrained contextual encoders, such as ELMo and BERT, has brought a great deal of interest in what these models learn: do they, without explicit supervision, learn to encode meaningful notions of linguistic structure? If so, how is this structure encoded? To investigate this, we introduce latent subclass learning (LSL): a modification to existing classifier-based probing methods that induces a latent categorization (or ontology) of the probe's inputs. Without access to fine-grained gold labels, LSL extracts emergent structure from input representations in an interpretable and quantifiable form. In experiments, we find strong evidence of familiar categories, such as a notion of personhood in ELMo, as well as novel ontological distinctions, such as a preference for fine-grained semantic roles on core arguments. Our results provide unique new evidence of emergent structure in pretrained encoders, including departures from existing annotations which are inaccessible to earlier methods.

==> tables_with_nmi.tex <==
\begin{table*}
\centering
\begin{tabular}{lrrrrr|rrrrrr}
\toprule
& \multicolumn{5}{c|}{Named Entities}
& \multicolumn{5}{c}{Universal Dependencies} \\
\midrule
                    & \textbf{P / R / F1}
                    & \hspace{-.1em}\textbf{\NMI}
                    & \hspace{-.1em}\textbf{Acc}
                    & \textbf{\DiversityShort$\uparrow$}
                    & \textbf{\UncertaintyShort$\downarrow$}
                    & \textbf{P / R / F1}
                    & \hspace{-.1em}\textbf{\NMI}
                    & \hspace{-.1em}\textbf{Acc}
                    & \textbf{\DiversityShort$\uparrow$}
                    & \textbf{\UncertaintyShort$\downarrow$} \\

\midrule
\textbf{Gold}       & 1.0 / 1.0 / 1.0
                    & 1.0  % NMI
                    & 1.0 & 9.71 & 1.00
                    
                    & 1.0 / 1.0 / 1.0  
                    & 1.0 % NMI
                    & 1.0 & 22.91 & 1.00 \\
\midrule
\textbf{Multi}      & .86 / .88 / .87           
                    & .60 % NMI
                    & .94 & 8.58 & 1.88 
                    
                    & .86 / .83 / .84           
                    & .64 % NMI
                    & .93 & 21.94 & 1.77 \\
\midrule
\textbf{LSL}        & .28 / .80 / .41           
                    & \textbf{.10} % NMI
                    & .96 & 2.85 & 1.45 

                    & .10 / .60 / .18
                    & .04 % NMI
                    & .94 & 3.50 & 2.07 \\

\textbf{\,+be}     & .20 / .43 / .27           
                    & .00 % NMI
                    & .96 & 4.78 & 31.23 
                    
                    & .18 / .13 / .15           
                    & .09 % NMI
                    & .94 & \textbf{29.83} & 12.33 \\

\textbf{\,+ie}     & .13 / 1.0 / .23  
                    & .00 % NMI
                    & .93 & 1.00 & \textbf{1.00}

                    & .09 / .79 / .15 
                    & .03 % NMI
                    & .94 & 2.00 & \textbf{1.01} \\

\textbf{\,+be+ie} & .43 / .54 / \textbf{.48} 
                    & .09 % NMI
                    & .88 &\textbf{7.00} & 1.10
                    
                    & .18 / .27 / \textbf{.22}
                    & \textbf{.10} % NMI
                    & .86 & 14.96 & 1.35 \\
\midrule
\textbf{Single}     & .13 / 1.0 / .23 
                    & .00 % NMI
                    & - & 1.00 & 1.00
                    
                    & .06 / 1.0 / .11
                    & .00 % NMI
                    & - & 1.00 & 1.00 \\
\bottomrule
\end{tabular}
\caption{
    Model selection results over BERT-large.
    \textbf{Multi} is the standard multi-class model trained directly on gold labels, and
    \textbf{Single} is the degenerate single-cluster baseline.
    %normalized mutual information is an especially difficult metric,
    Our clustering regularizers (\textbf{b}atch and/or \textbf{i}nstance-level \textbf{e}ntropy), when taken together, yield a good tradeoff between \textbf{div}ersity and \textbf{unc}ertainty,
    while maintaining appreciable \NMI{} (though it is a difficult metric),
    with some expense to binary classification \textbf{acc}uracy. 
}
\label{tab:model-selection-results}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{l|rrr|rrr|rrr|r}


\toprule
     & \multicolumn{3}{|c|}{\textbf{BERT-lex}}
     & \multicolumn{3}{|c|}{\textbf{ELMo}}
     & \multicolumn{3}{|c|}{\textbf{BERT-large}}
     & \multicolumn{1}{|c }{\textbf{Gold}}
     \\
\midrule
\textbf{Task}
    & P / R / F1
    & \hspace{-.6em}\NMI{}
    & \hspace{-.4em}\DiversityShort
    & P / R / F1
    & \hspace{-.6em}\NMI{}
    & \hspace{-.4em}\DiversityShort
    & P / R / F1
    & \hspace{-.6em}\NMI{}
    & \hspace{-.4em}\DiversityShort
    & \hspace{-.4em}\DiversityShort
    \\
\midrule

\textbf{Deps}
    & .06 / .86 / .11
    & .00
    & 1.33
    & .23 / .42 / \textbf{.29}
    & \textbf{.12}
    & 11.11
    & .14 / .33 / .19
    & .07
    & \textbf{11.22}
    & 22.91
    \\
%\textbf{Deps (undir.)}
%    & .09 / .54 / .16
%    & .04
    %& .??
%    & .19 / .23 / .21
%    & \textbf{.11}
    %& .??
%    & .23 / .23 / \textbf{.23}
%    & .10
%    & 18.51
%    & 22.91
%    \\
\textbf{Entities}
    & .19 / .39 / .26
    & .01
    & 4.33
    & .40 / .66 / \textbf{.50}
    & .13
    & 5.07
    & .47 / .53 / \textbf{.50}
    & \textbf{.20}
    & \textbf{7.50}
    & 9.71
    \\
\textbf{Nonterm.}     
    & .22 / .80 / .34
    & .01
    & 1.47
    & .36 / .25 / .30
    & .13
    & \textbf{10.16}
    & .35 / .34 / \textbf{.35}
    & \textbf{.20}
    & 7.80
    & 7.15
    \\
\textbf{Roles}   
    & .19 / .39 / \textbf{.26}
    & .00
    & 2.81
    & .40 / .17 / .24
    & \textbf{.08}
    & \textbf{22.35}
    & .37 / .17 / .24 
    & .07
    & 18.70 
    & 8.73 
    \\
%\textbf{Relations}        
%    & .07 / .97 / .13
%    & .00
%    & .11 / .78 / .20
%    & \textbf{.05}
%    & .16 / .63 / \textbf{.25}
%    & \textbf{.05}
%    & 3.87 
%    & 24.78 
%    \\

\bottomrule
\end{tabular}
\caption{Results by task for three pretrained encoding methods.
All probing models were trained with the LSL loss and cluster regularization coefficients \( \alpha = \beta = 1.5 \),
and chosen by the best-of-5 consistency criterion and detailed in \autoref{sec:model-selection}.
Uncertainty for all models was close to 1 and is omitted for space.}
%For each hyperparameter setting, the latently learned classes were fairly stable,
%with an average pairwise F1 of \TODO{XX} between models in the same group.
%In 63\% of cases, the model selected by our consistency criterion
%had the highest F1-score with respect to gold in its group.
\label{tab:full-experiment-results}
\end{table*}
